Variational Learning ISTA

Compressed sensing combines the power of convex optimization techniques with a sparsity-inducing prior on the signal space to solve an underdetermined system of equations. For many problems, the sparsifying dictionary is not directly given, nor its existence can be assumed. Besides, the sensing matrix can change across different scenarios. Addressing these issues requires solving a sparse representation learning problem, namely dictionary learning, taking into account the epistemic uncertainty of the learned dictionaries and, finally, jointly learning sparse representations and reconstructions under varying sensing matrix conditions. We address both concerns by proposing a variant of the LISTA architecture. First, we introduce Augmented Dictionary Learning ISTA (A-DLISTA), which incorporates an augmentation module to adapt parameters to the current measurement setup. Then, we propose to learn a distribution over dictionaries via a variational approach, dubbed Variational Learning ISTA (VLISTA). VLISTA exploits A-DLISTA as the likelihood model and approximates a posterior distribution over the dictionaries as part of an unfolded LISTA-based recovery algorithm. As a result, VLISTA provides a probabilistic way to jointly learn the dictionary distribution and the reconstruction algorithm with varying sensing matrices. We provide theoretical and experimental support for our architecture and show that our model learns calibrated uncertainties.

==> sections/abstract.tex <==
Compressed sensing combines the power of convex optimization techniques with a sparsity-inducing prior on the signal space to solve an underdetermined system of equations. For many problems, the sparsifying dictionary is not directly given, nor its existence can be assumed. Besides, the sensing matrix can change across different scenarios. Addressing these issues requires solving a sparse representation learning problem, namely dictionary learning, taking into account the epistemic uncertainty of the learned dictionaries and, finally, jointly learning sparse representations and reconstructions under varying sensing matrix conditions.
We address both concerns by proposing a variant of the LISTA architecture. First, we introduce \ac{A-DLISTA}, which incorporates an augmentation module to adapt parameters to the current measurement setup. Then, we propose to learn a distribution over dictionaries via a variational approach, dubbed \ac{VLISTA}. \ac{VLISTA} exploits A-DLISTA as the likelihood model and approximates a posterior distribution over the dictionaries as part of an unfolded LISTA-based recovery algorithm. 
As a result, \ac{VLISTA} provides a probabilistic way to jointly learn the dictionary distribution and the reconstruction algorithm with varying sensing matrices. We provide theoretical and experimental support for our architecture and show that our model learns calibrated uncertainties.



%\textcolor{blue}{(Possible) TODOs:}

%\begin{itemize}
%    \item \textcolor{blue}{SSIM as a function of the number of layers for LISTA models - Appendix}
%    \item \textcolor{blue}{Improve explanation why to choose standard gaussian as first prior for VLISTA instead of learned $\mu$ and $\sigma$}
%    \item \textcolor{blue}{Add reference to inpainting task description specifically concerning the masking of pixels}
%    \item \textcolor{blue}{Explain why with a higher SNR OD and IID are more overlapped - might look counterintuitive}
%\end{itemize}


==> tables/complexity_analysis_par_time.tex <==
\begin{table}[!b]
\caption{Number of trainable parameters (Millions) and Average inference time (milliseconds) for different models. Concerning the inference time, we report the average value with its error considering 10 and 50 measurements setups.} \label{tab:params_time}
\begin{center}
\begin{threeparttable}
\begin{tabularx}{\linewidth}{@{}ll|YYY@{}}
\toprule
&\multirow{2}{*}{} & \multicolumn{1}{c}{Parameters $(M)$} & \multicolumn{2}{c}{Average Inference Time $(ms)$} \\ \cline{4-5}
&\multirow{2}{*}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{meas. = 10} & \multicolumn{1}{c}{meas. = 500}\\
\midrule
&\multicolumn{1}{l|}{ISTA} & $0.00$ & $54.0_{\pm0.6}$ (norm: $41.5_{\pm0.6}$) & $(1.55_{\pm0.02})e^3$ (norm.: $(1.53_{\pm0.02})e^3$) \\  
&\multicolumn{1}{l|}{NALISTA${}^1$} & $3.33e^{-1}$ & $5.8_{\pm0.2}$ & $7.0_{\pm0.3}$ \\ 
&\multicolumn{1}{l|}{LISTA} & $3.15$ & $1.1_{\pm0.1}$ & $1.5_{\pm0.3}$ \\  
% &\multicolumn{1}{l|}{A-DLISTA${}^{2,4}$ (shared)} & $3.15$ (Aug. NN: $3.11e^{-3}$) & $1.05$ (Aug. NN: $4.03e^{-3}$) & $19.3_{\sigma=8.7}$ \\ 
&\multicolumn{1}{l|}{A-DLISTA${}^{2}$} & $3.15$ (Aug. NN: $3.11e^{-3}$) & $8.2_{\pm0.3}$ &  $9.1_{\pm0.5}$ \\  % Not shared
\midrule
&\multicolumn{1}{l|}{VLISTA} & $3.13^\dagger$ & $19.7_{\pm0.4}^\dagger$ &  $21.3_{\pm0.4}^\dagger$ \\ 
\midrule
\multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{VLISTA}}}
&\multicolumn{1}{l|}{Prior Model} & $1.10$ & $-$ &  $-$ \\   
&\multicolumn{1}{l|}{Posterior Model} & $2.08$ & $3.6_{\pm0.2}^\ddagger$ &  $4.1_{\pm0.2}^\ddagger$ \\ 
&\multicolumn{1}{l|}{Likelihood Model} & $1.05$ & $2.7_{\pm0.2}^\ddagger$ &  $3.05_{\pm0.2}^\ddagger$ \\  
\bottomrule
\end{tabularx}
\begin{tablenotes}
\item[1] LSTM hidden size equal to 256; 
\item[2] Each layer learns its own dictionary; 
\item[$\dagger$] Full model at inference - Prior model NOT used; 
\item[$\ddagger$] Single iteration.
\end{tablenotes}
\end{threeparttable}
\end{center}
\end{table}

==> tables/synth_quntiles_meas.tex <==
\begin{table}[!ht]
\caption{NMSE's median (the lower the better) for different number of measurements. Top five rows concern non-Bayesian models whilst the bottom two report results for Bayesian approaches. For each of the two set of results, we highlight in bold the best performance.}

\label{tab:quantiles_synth_measurements}
\begin{center}
% \begin{threeparttable}
\begin{tabularx}{\linewidth}{@{}lcccccc@{}}
\toprule

\multirow{2}{*}{} & \multicolumn{6}{c}{Q=0.5 $\downarrow$} \\
\multirow{2}{*}{} & \multicolumn{6}{c}{} \\
\multirow{2}{*}{} & \multicolumn{6}{c}{number of measurements} \\ \cline{2-7}
\multirow{2}{*}{} & 10 & 100 & 200 & 300 & 400 & 500 \\ 
\midrule

% \multirow{10}{*}{\STAB{\rotatebox[origin=c]{90}{\small{Non-Bayes}}}}
\multicolumn{1}{l|}{ISTA} & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$\\

% %& \multicolumn{1}{l|}{\ac{ISTA}$^{\dagger}$} & +0.38 & +0.05 & -0.13 & -1.90 & -3.28 \\
% %& \multicolumn{1}{l|}{\ac{ISTA}$^{\dagger}$ (1000 iterations)} & +0.01 & -0.04 & -1.62 & -8.30 & -15.76 \\

% & \multicolumn{1}{l|}{\ac{LISTA}} & -0.01 & -1.60 & -1.28 & -2.82 & -4.37 \\
\multicolumn{1}{l|}{\ac{LISTA}} & $-0.45e^{-2}$ & $-1.15e^{-1}$ & $-0.61$ & $-1.31$ & $-1.70$ & $-2.12$\\

% & \multicolumn{1}{l|}{\ac{ALISTA}} & &  & &  &  \\
\multicolumn{1}{l|}{\ac{ALISTA}} & $+0.11e^{-2}$ & $-0.35e^{-1}$ & $-0.30$ & $-0.36$ & $-0.94$ & $-0.99$ \\

% & \multicolumn{1}{l|}{\ac{NALISTA}} & & & &  &  \\
\multicolumn{1}{l|}{\ac{NALISTA}} & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$\\

% & \multicolumn{1}{l|}{\ac{DLISTA}}  & -3.12 & -5.22 & -7.18 & -10.62  & -17.92  \\
\multicolumn{1}{l|}{\ac{DLISTA}} & $-1.34e^{-2}$ & $-3.05e^{-1}$ & $-0.86$ & $-1.19$ & $-1.65$ & $-1.90$ \\

% & \multicolumn{1}{l|}{\ac{A-DLISTA} (our)}  & \bf -5.45 & \bf -14.82 & \bf -20.91 & \bf -19.47 & \bf -22.35  \\
\multicolumn{1}{l|}{\ac{A-DLISTA}} & $-1.55e^{-2}$ & $-5.96e^{-1}$ & $-1.31$ & $-1.86$ & $-2.33$ & $-2.72$ \\

 \midrule

% \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\small{Bayes}}}}
% & \multicolumn{1}{l|}{\ac{BCS}} & +0.16 & +0.17 & +1.91 & +2.34 & +2.55 \\
\multicolumn{1}{l|}{\ac{BCS}} & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$\\

% & \multicolumn{1}{l|}{\ac{VLISTA} (our)} & \bf -3.67 & \bf -8.20 & \bf -13.94 & \bf -15.31 & \bf -14.02 \\
\multicolumn{1}{l|}{\ac{VLISTA}} & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$ & $(\pm)e^{-}$\\

\bottomrule

\end{tabularx}

% \end{threeparttable}

\end{center}

\end{table}

